The Hitchiker's Guide to Successful Living Lab Operations

Living labs have been established across different countries to evaluate how the interaction between humans and buildings can be optimized to improve comfort, health, and energy savings. However, existing living labs can be too project-specific, not scalable, and inflexible for comparison against other labs. Furthermore, the lack of transparency in its software infrastructure inhibits opportunities for critique and reuse, reducing the platform's overall potential. In the face of climate change and global energy shortage, we envision the future of living labs to be open source and scalable to support the integration of different IoTs, subjective measures, human-building interactions, security, and privacy contexts. In this work, we share our living lab software stack and present our experience developing a platform that supports qualitative and quantitative experiments from the ground up. We propose the first open-source interoperable living lab platform for multidisciplinary smart environment research.

==> tables/device_table.tex <==
\begin{longtable}[c]{cp{2in}p{3in}} % <-- Replaces \begin{table}, alignment must be specified here (no more tabular)
  \caption{Device Descriptions}
  \label{tab:table1}\\
  \toprule
  \hline
  \textbf{Abbreviation} & \textbf{Model} &\textbf{Description}\\
  \midrule
  \endfirsthead % <-- This denotes the end of the header, which will be shown on the first page
  \endhead % <-- Everything between \endfirsthead and \endhead will be shown as a header on every page
    \hline
    AW & Awair V2 & AWAIR  monitors fine dust particulates—or PM2.5 levels, as well as CO2 , VOC’s, plus temperature and humidity.\\

    CO &  60.CO2 SLR TMP HUM  & The Pressac Sensing wireless CO2 Sensor is designed to measure and report levels of Carbon Dioxide, ambient temperature and relative humidity in an internal environment. \\

    DS & Wireless Door/Window Sensor ExT-MDCCP & Provides wireless status of windows and/or doors using a magnet contact switch that is powered by a solar cell. \\

    DTMS & Dual Tech Ceiling Mount Sensor MOS-DT & The Dual Tech Ceiling Mount Sensor (MOSDT) is a 360 degree ceiling sensor that procides battery-free wireless occupancy detection that uses a combination of passive infrared (PIR) and audio sensing technologies ensures positive occupant detection. \\

    BC & Estimoe Location Beacons & In combination with an app, Estimotes can provide  approximate location data with the consent of the users \\
  
    LL & Enocean ELLSU-W-EO Light Level Sensor & Measures and reports the level of available natural light.\\

    PB & Power Blade & An AC plug-load meter that measures real, reactive and apparent power, and reports this data, along with cumulative energy consumption, over an industry-standard Bluetooth Low Energy radio \cite{debruin2015powerblade}\\

    TH & Pressac Mini Temperature And Humidity Sensor & A fully wireless, solar powered compact sensor to measure temperature and humidity\\
    \hline
    \bottomrule
\end{longtable}
   %Table or figure


==> tables/device_table_brad.tex <==
\begin{table}[]
\small
\begin{tabulary}{\linewidth}{|L|p{7.5cm}|L|}
\hline
   Sensor Type  & Data Stream & Privacy Concerns          \\ \hline

% \multirow{6}{*}{\STAB{\rotatebox[origin=c]{90}{Environmental}}} & 
\multicolumn{3}{|c|}{Environmental} \\ \hline
Temperature & Celsius & Low     \\ 
Humidity & percent & Low                                        \\ 
Illuminance Level (Light) & Lux & Low                             \\ 
Air Quality & VOC, CO2, PM 2.5 & Low                             \\ 
Motion sensor & Boolean & Low/medium                             \\ 
Door/window open & Boolean & Low           \\ \hline

\multicolumn{3}{|c|}{Human} \\ \hline
% \multirow{5}{*}{\STAB{\rotatebox[origin=c]{90}{Human}}} &
Smartwatch & Step Count, Heart-rate, Skin temperature, GSR, Noise level & High     \\ 
Mobile phones & GPS, App use, calendar & High                            \\ 
Desk Camera \& Image Processing & Perceived emotion, facial landmarks   & High                             \\ 
Bluetooth Beacons & Location tracking & High                              \\ 
Surveys & productivity, mood, physical and social activity & High         \\ \hline

\multicolumn{3}{|c|}{Operational} \\ \hline
% \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{Operational}}} &
Appliance energy consumption & Watts & High     \\ 
Circuit energy consumption & Watts & Medium                             \\ 
Water consumption & Gallons   & Low                             \\ \hline
\end{tabulary}
\caption{\small Living Link Lab data streams.}
\label{table:lll-streams}
\end{table}


==> tables/living_labs_save <==
% \begin{landscape}
% \onecolumn
\begin{longtable}{>{\raggedright}p{1in}>{\raggedright}p{0.75in}p{0.75in}p{0.75in}p{0.75in}p{0.75in}p{0.75in}}
    \caption{List of living labs constructed after 2000, with infrastructure open-sourced (adopted \cite{cureau2022bridging}). We were not able to find implementations that were readily accessible}
    \label{tab:lls}
    \hline
    \textbf{Name} & \textbf{Country} & \textbf{Source Code Accessible} & \textbf{Surveys Deployed} & \textbf{Sensors Deployed}  & \textbf{Study Duration} & \textbf{Reference} \\
    \hline
    \hline
    BNZEB & Italy & N/A & N & Y & 1+ years & \cite{ascione2020nearly,ascione2019framework}\\ %The nature of the BNZEB as laboratory implies presence of a number of sensors, meters, availability of monitoring of thermal, acoustic and lighting performances like no other buildings in Italy.
    \hline
    % CARBSE Net Zero Energy Building at CEPT University & France & N & ?\\
    Carleton University Buildings & Canada & N/A & N & Y & 15 months, 7-12 months, 1 month preliminary data collection + 9 weeks study,  & \cite{gilani2018preliminary, gunay2017development,bursill2020multi,gunay2018development}\\
    \hline
    % CELLS & Switzerland & ? & ? & ? & ? & ?\\ #No paper found
    CIRIAF Offices & Italy & N/A & Y & Y Lux Meter, Amp Meter, Air Temp, Window/Door opening & 1 Yr and 2Yrs & \cite{piselli2019occupant,pisello2016peers}\\
    \hline
    ComfortSense Project & Italy & N/A & N & ? & ? & \cite{cottafava2019crowdsensing}\\
    \hline
    David Bower Center \footnote{\cite{roa2020targeted} has a similar open source occupancy survey distribution?} & California, USA & A & Y & Y temperature & 14 months (Oct 20 through Dec 10, 2019) & \cite{roa2020targeted}\\
    \hline
    ENERGISE Living Labs & Denmark, Finland, Germany, Hungary, Ireland, Switzerland, the Netherlands, and United Kingdom & N/A & Y & Thermo-loggers  households filling in the surveys \footnote{potentially due to loggers being placed differently in the room} & 9 month & \cite{sahakian2021challenging}\\
    & & ? & ? & ? & 8 months & \cite{laakso2021towards}\\
    \hline
    House Living Labs Project & Australia & N/A & N & Internal temperature, Gas, Photovoltaic electricity generation & 1 + Years, Dec2014 - 2015 & \cite{eon2018influence}\\
    \hline
    % Nordhavan living labs & Denmark & ? & ? & ? & ? & \cite{christensen2020demand}\\
    % \hline
    % % NREL's Research Support Facility (RSF) & Colorado, USA & ? & ? & ? & ?\\ # No paper
    % % \hline
    % % Odoo project & Hungary & ? & ? & ? & ? & ?\\ # No paper
    % % \hline
    % Passivhaus in Italy & Italy & ? & ? & ? & ? & \cite{causone2019yearly}\\
    % \hline
    % Sant'Appollinare Building & Italy & ? & ? & ? & ? & \cite{piselli2020integrated}\\
    % \hline
    Sutardja Dai Hall at University of California, Berkeley & California, USA & N & N & Y & Two weekend days &  \cite{ma2011optimal}\\
    \hline
    Well Living Lab & Minnesota, USA & N & Y & Y \footnote{Notably, has a description track sensor failure. They also note the importance to 1) reduce spatial variability between desk-level environmental conditions so that inter-cohort variability in exposure is reduced} & N/A & \cite{clements2019spatial}\\
    & & N & Y\footnote{Daily and weekly surveys with interviews} & Y\footnote{Combines acoustic, lighting, and thermal conditions} & 18 weeks & \cite{jamrozik2018novel}\\
    & & N & Y\footnote{Morning–Eveningness Questionnaire (MEQ)} & Y\footnote{Lighting, thermal, accoustics, air quality; includes the empatica wearable} & 4 weeks & \cite{zhang2020impacts}\\
    & & N & Cost-Effective Open Plan Environments (COPE) and SBS & Y (same sensors as above) & 14 weeks & \cite{jamrozik2019access}\\
    & & N & ? & ? & ? & \cite{aristizabal2021biophilic}\\
    \hline
    % ZEB Laboratory & Norway & ? & ? & ? & ? & ?\\ # Does not exist
    % \hline
    ZEB Living Lab & Norway & N & N & Y (LabView \cite{krauss1999labview}) & N/A \footnote{description of the test facility, but not of any specific study}) & \cite{goia2015zeb}
    % \\
    % & & ? & ? & ? (LabView \cite{krauss1999labview}) & N/A \footnote{description of the test facility, but not of any specific study}) & \cite{woods2019homemaking}\\
    % & & ? & ? & ? &  & \cite{jurisoo2018beyond}\\
    \hline
\end{longtable}
\twocolumn
% \end{landscape}
